DreamHOI: Subject-Driven Generation of 3D Human-Object Interactions with Diffusion Priors

We present DreamHOI, a novel method for zero-shot synthesis of human-object interactions (HOIs), enabling a 3D human model to realistically interact with any given object based on a textual description. This task is complicated by the varying categories and geometries of real-world objects and the scarcity of datasets encompassing diverse HOIs. To circumvent the need for extensive data, we leverage text-to-image diffusion models trained on billions of image-caption pairs. We optimize the articulation of a skinned human mesh using Score Distillation Sampling (SDS) gradients obtained from these models, which predict image-space edits. However, directly backpropagating image-space gradients into complex articulation parameters is ineffective due to the local nature of such gradients. To overcome this, we introduce a dual implicit-explicit representation of a skinned mesh, combining (implicit) neural radiance fields (NeRFs) with (explicit) skeleton-driven mesh articulation. During optimization, we transition between implicit and explicit forms, grounding the NeRF generation while refining the mesh articulation. We validate our approach through extensive experiments, demonstrating its effectiveness in generating realistic HOIs.

==> sec/scratch.tex <==
\section{Methods}
\label{sec:methods}

\begin{algorithm}
\caption{Main algorithm}\label{alg:main}
\begin{algorithmic}
    \Require Mesh $M$ of the object, semantic relation $r$
    \State Train NeRF $\theta_0$ modeling a human in relation $r$ with $M$ using SDS
    \State Fit a human model $\xi_0$ from $\theta_0$
    \For {$t=1,\ldots,T$}
        \State Initialize DMTet $\theta_{t}$ from the mesh of $\xi_{t-1}$
        \State Train DMTet $\theta_{t}$ modeling a human in relation $r$ with $M$ using SDS
        \State Fit a human model $\xi_{t}$ from $\theta_{t}$
    \EndFor
    \State \Return $\xi_T$
\end{algorithmic}
\end{algorithm}

Our final loss gradient for optimizing $\theta_0$ is
\begin{multline} \label{eq:loss}
\nabla_\theta\mathcal{L}=\lambda_{\text{SDS}}\nabla_\theta\mathcal{L}_{\text{SDS}}(\varphi,\bm x,y)
\\ {}+
\lambda_{\text{SDS},h}\nabla_\theta\mathcal{L}_{\text{SDS}}(\varphi_h,\bm x_h,y_h)
\\ {}+\lambda_{\text{MO}}\nabla_\theta\mathcal{L}_{\text{MO}}
+\lambda_{\text{I}}\nabla_\theta\mathcal{L}_{\text{I}}
+\lambda_{\text{S}}\nabla_\theta\mathcal{L}_{\text{S}}
\end{multline}
where $\lambda_-$, $\mathcal{L}_-$ are hyperparameters and additional loss terms (below), $\varphi_h$ is a (potentially different) diffusion model for supervision of the human-only rendering, and the prompts are as follows for the example $r$ being ``sitting'' on ball $M$:
\begin{enumerate}
\item $y$ is ``A photo of a person sitting on a ball''.
\item $y_h$ is ``A photo of a person sitting'' with negative prompt ``ball''.
\end{enumerate}
In experiments, we set $\varphi$ to weights of DeepFloyd IF~\cite{???}, because it has a large text encoder (namely, T5 v1.1 XXL~\cite{raffel2023exploringlimitstransferlearning}) that empirically can better understand the semantic relation $r$ (see~\TODO{2D experiments in supplementary}). We set ${\varphi_h}$ to a mixture between MVDream~\cite{shi2024mvdreammultiviewdiffusion3d} and DeepFloyd IF for training the human NeRF, because empirically MVDream is more effective in consistent and stable 3D generation and in solving the multi-face Janus problem, and DeepFloyd can understand prompts to avoid a degenerate human model (overly simplistic, not photo-realistic, missing limbs, \etc).

One problem frequently encountered in generation is that the human NeRF $f_{\theta_0}$ is encouraged to produce a layer that covers the mesh $M$. This might distort or displace $M$ so the generated human pose might not be accurate. To counter this, we added the negative prompt in $y_h$ above, which we found to reduce this problem. We also include two additional loss terms:
\begin{equation}
\mathcal{L}_{\text{MO}}=\text{mean}_{\text{$R$:$R$ intersects $M$}}(1-w_I)
\end{equation} penalizes \emph{mesh occlusion} by the NeRF and
\begin{equation}
\mathcal{L}_{\text{I}}=\text{mean}_{R,i:\text{$\bm\mu_i$ is inside $M$}}\tau_i
\end{equation} penalizes \emph{intersection} between the NeRF and the inside of $M$. Finally, a thin or partial covering of $M$ by the NeRF has little impact on the human model prediction in the next stage.

We also include
\begin{equation}
\mathcal{L}_{\text{S}}=\text{mean}_{R}\sum_iw_i
\end{equation}
which encourages \emph{sparsity} of the rendered NeRF as in~\cite{threestudio}, so that it does not expand and fill the entire space.

% TODO
We also found it important to tune the prompts and negative prompts, additional losses, and the sampling of time steps $t$. \TODO{see experiments/supplementary}



\subsection{DMTet Training}
The reason we \emph{do not directly optimize the SMPL weights $\xi_t$ using SDS} is that it never works in our experiments (see~\TODO{supplementary}). Instead, we follow an iterative approach by optimizing a DMTet $f_{\theta_{t}}$ initialized from the SMPL model $\xi_{t-1}$ using SDS, and then re-fitting a SMPL model $\xi_{t}$ to the trained DMTet $f_{\theta_{t}}$.

Formally, we follow the setup of Magic3D~\cite{lin2023magic3dhighresolutiontextto3dcontent}: $f_{\theta_{t}}$ consists of a tetrahedral grid $T$, with vertices in the grid $\bm v_i \in V_T$ and associated signed distance value $s_i\in\mathbb{R}$ and deformation from initial position $\Delta\bm v_i\in\mathbb{R}^3$. It is rendered by extracting a mesh using the differentiable marching tetrahedra algorithm~\cite{shen2021dmtet}. The mesh is colored using an MLP network $(x,y,z)\mapsto\bm c\in\mathbb{R}^3$, which is initialized by making it approximate a fixed texture for SMPL models such as~\cite{smpl_texture_github}. This mesh is merged with $M$, then rendered by a differentiable rasterizer~\cite{laine2020modularprimitiveshighperformancedifferentiable_nvdiffrast} and composited with the background (from an MLP similar to~\cref{sec:nerf-train}) with anti-aliasing to produce image $\bm x$.

For training $f_{\theta_t}$, we largely follow the steps used to train NeRF (\cref{sec:nerf-train}). We apply the SDS loss $\nabla_\theta\mathcal{L}_{\text{SDS}}$ from~\cref{eq:sds-loss} to the rendered result. We omit other losses (``human-only'' SDS loss, mesh occlusion, intersection, and sparsity), as we found them unnecessary because the geometry of the DMTet is already initialized to be near our intended solution. We also perform shading when rendering as in~\cite{poole2022dreamfusiontextto3dusing2d,lin2023magic3dhighresolutiontextto3dcontent} for a more fine-grained result and to reduce surface artifacts. Following Magic3D~\cite{lin2023magic3dhighresolutiontextto3dcontent}, we lower the sample space of $t$ to $t\sim\mathcal{U}(0.02,0.5)$, and increase the rendering resolution to $512\times512$.

\subsection{Discussions}

\paragraph{Motivation for the pipeline.}
From a 3D generation perspective, our approach is similar to the coarse-to-fine pipeline of Magic3D~\cite{lin2023magic3dhighresolutiontextto3dcontent}, initializing and training a NeRF in the coarse stage and converting it to a DMTet which is further refined. However, our human model prediction stage between the two stages effectively \emph{grounds} the generation to be realistic and human-like. Moreover, our final output is the predicted human model parameters $\xi_T$ instead of a NeRF, mesh, or DMTet, which is much more useful and versatile in further applications of 3D human generation.

Using a DMTet as the next stage has the added benefit that it is easy to initialize from an existing mesh or signed distance function (SDF), which is why our pipeline supports SMPL naturally as well as other models.

From a pose estimation perspective, whereas previous works focus on estimating a human pose given, say, views of the scene, our method generates a human pose by directly supplying the views from a 3D generation method. Unfortunately, the straightforward approach of training pose parameters directly using SDS does not work, because of the locality of gradients (\TODO{}) which necessitates our method.

\paragraph{Mixture of guidances.}
Unlike previous works, we adopt a mixture of SDS losses from multiple guidance models (namely, MVDream and DeepFloyd IF). As explained in~\cref{sec:nerf-train}, each model has its benefits: MVDream enables view-consistent 3D generation and DeepFloyd IF has a deep text encoder, and we found through initial experiments that only a mixture could achieve the best of both worlds. We suspect a future unified model that has both a large text encoder and is specialized to 3D generation and/or more specialized hyperparameter, prompt tuning, and loss terms can eliminate the need of this mixture and reduce engineering and tuning costs, but as of now this mixture achieves our goals the best.

\paragraph{Choice of $T$.}  % maybe belongs to experiments section
In practice, we find $T=0$ (no re-fitting) already produces quite consistent results, but $T>0$ fixes the following problems:
\begin{enumerate}
\item Missing limbs, \eg limbs inside $M$
\item Misplaced details, \eg hands slightly off the handle
\item NeRF covering $M$
\item The multi-face Janus problem, \eg a person kicking with the left leg in one view and the right leg in another \TODO{show in figure}
\end{enumerate}

